Generating Counterfactual Explanations Under Temporal Constraints

Counterfactual explanations are one of the prominent eXplainable Artificial Intelligence (XAI) techniques, and suggest changes to input data that could alter predictions, leading to more favourable outcomes. Existing counterfactual methods do not readily apply to temporal domains, such as that of process mining, where data take the form of traces of activities that must obey to temporal background knowledge expressing which dynamics are possible and which not. Specifically, counterfactuals generated off-the-shelf may violate the background knowledge, leading to inconsistent explanations. This work tackles this challenge by introducing a novel approach for generating temporally constrained counterfactuals, guaranteed to comply by design with background knowledge expressed in Linear Temporal Logic on process traces (LTLp). We do so by infusing automata-theoretic techniques for LTLp inside a genetic algorithm for counterfactual generation. The empirical evaluation shows that the generated counterfactuals are temporally meaningful and more interpretable for applications involving temporal dependencies.

==> misc.tex <==
%Example with outcome included


\begin{subfigure}{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{
$\trace_1 = \submitapplication, \automaticcheck, \manualcheck, \informphone, \accept, \createoffer, \informphone, \askappointment \quad \color{red}{\text{(No Agr.)}}$
}
\caption{The ongoing trace with a negative outcome.}
\label{subfig:trace}
\end{subfigure}\\[5pt]
\begin{subfigure}{\columnwidth}
\centering
\resizebox{\columnwidth}{!}{
$\begin{aligned}
\trace_{c1} & = \submitapplication, \wrongtask{\manualcheck}, \wrongtask{\automaticcheck}, \informphone, \accept, \createoffer, \informphone, \senddocument \quad \color{teal}{\text{(Agr. reached)}} \\
\trace_{c2} & = \submitapplication, \automaticcheck, \manualcheck, \informphone, \accept, \createoffer, \informphone, \senddocument \quad \color{teal}{\text{(Agr. reached)}} \\
\trace_{c3} & = \submitapplication, \automaticcheck, \wrongtask{\informphone}, \accept, \createoffer, \wrongtask{\informsms}, \senddocument \quad \color{teal}{\text{(Agr. reached)}} \\
\trace_{c4} & = \submitapplication, \automaticcheck, \informphone, \informphone, \accept, \createoffer, \informphone, \senddocument, \askappointment \quad \color{teal}{\text{(Agr. reached)}} \\
\trace_{c5} & = \submitapplication, \automaticcheck, \manualcheck, \wrongtask{\informphone}, \accept, \createoffer, \wrongtask{\informemail}, \senddocument \quad \color{teal}{\text{(Agr. reached)}}
\end{aligned}$
}
\caption{Examples of counterfactual traces with a positive outcome.}
\label{subfig:counterfactuals}
\end{subfigure}\\[5pt]

%%%%% OLD TABLE
\begin{table*}[t]
\centering
{\fontsize{9pt}{10pt}\selectfont
\scalebox{0.75}{
\begin{tabular}{llccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{$\frac{|\tasks_\varphi|}{|\tasks|}$}  &  & \multicolumn{5}{c}{Claim Management} & \multicolumn{5}{c}{BPIC2012} &  \multicolumn{5}{c}{BPIC2017}  \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17}
 & & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort  & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur \\
\midrule
 \multirow{6}{*}{10\%} 
& Dist &
 $\winner{0.42}\rank{1}$ & $0.48\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ &%SYNTH
 $\winner{0.47}\rank{1}$ & $0.54\rank{5}$ & $0.50\rank{2}$ & $\winner{0.47}\rank{1}$ & $0.50\rank{2}$ &%BPIC2012
 $0.58\rank{4}$ & $0.59\rank{4}$ & $0.50\rank{2}$ & $\winner{0.44}\rank{1}$ & $0.50\rank{2}$ \\ %BPIC17
& Spars &
 $\winner{2.18}\rank{1}$ & $2.50\rank{2}$ & $2.58\rank{2}$ & $2.63\rank{2}$ & $2.58\rank{2}$ &%SYNTH
 $\winner{6.83}\rank{1}$ & $7.69\rank{5}$ & $\winner{6.95}\rank{1}$ & $\winner{6.79}\rank{1}$ & $\winner{6.97}\rank{1}$ &%BPIC2012
 $6.75\rank{4}$ & $6.95\rank{4}$ & $\winner{5.60}\rank{1}$ & $\winner{5.20}\rank{1}$ & $5.85\rank{3}$ \\%BPIC17
& Plaus &
 $9.11\rank{2}$ & $\winner{8.49}\rank{1}$ & $8.88\rank{2}$ & $8.84\rank{2}$ & $8.92\rank{2}$ &%SYNTH
 $8.15\rank{5}$ & $\winner{7.49}\rank{1}$ & $\winner{7.37}\rank{1}$ & $\winner{7.26}\rank{1}$ & $\winner{7.38}\rank{1}$ &%BPIC2012
 $7.62\rank{5}$ & $\winner{7.51}\rank{1}$ & $\winner{6.81}\rank{1}$ & $\winner{6.59}\rank{1}$ & $\winner{6.86}\rank{1}$ \\%BPIC17
& Conf &
 $0.77\rank{5}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
 $0.74\rank{5}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
 $0.86\rank{5}$ & $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dive &
 $0.46\rank{4}$ & $0.48\rank{4}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ &%SYNTH
 $\winner{0.41}\rank{1}$ & $0.35\rank{5}$ & $\winner{0.40}\rank{1}$ & $\winner{0.41}\rank{1}$ & $\winner{0.40}\rank{1}$ &%BPIC2012
 $\winner{0.63}\rank{1}$ & $0.58\rank{2}$ & $0.49\rank{3}$ & $0.44\rank{5}$ & $0.49\rank{3}$ \\ %BPIC17
& Run &
 $\winner{1.0}\rank{1}$ & $2.53\rank{2}$ & $4.65\rank{5}$ & $4.38\rank{3}$ & $4.09\rank{3}$ &%SYNTH
 $\winner{2.5}\rank{1}$ & $25\rank{4}$ & $90\rank{5}$ & $12\rank{2}$ & $17\rank{3}$ &%BPIC2012
 $\winner{5.1}\rank{1}$ & $29.1\rank{2}$ & $78.3\rank{3}$ & $57.3\rank{3}$ & $65.5\rank{3}$ \\%BPIC17
\midrule
\multirow{6}{*}{25\%} 
& Dist &
 $\winner{0.42}\rank{1}$ & $0.48\rank{2}$ & $0.47\rank{2}$ & $0.50\rank{5}$ & $0.47\rank{2}$ &%SYNTH
 $0.44\rank{4}$ & $0.47\rank{2}$ & $0.38\rank{4}$ & $\winner{0.30}\rank{1}$ & $0.36\rank{2}$ &%BPIC2012
 $0.55\rank{4}$ & $0.58\rank{4}$ & $0.33\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.31\rank{2}$ \\%BPIC17
& Spars &
 $\winner{2.19}\rank{1}$ & $2.50\rank{2}$ & $2.45\rank{2}$ & $2.58\rank{5}$ & $2.42\rank{2}$ &%SYNTH
 $6.38\rank{3}$ & $7.01\rank{3}$ & $5.24\rank{3}$ & $\winner{4.38}\rank{1}$ & $4.92\rank{2}$ &%BPIC2012
 $6.47\rank{4}$ & $6.77\rank{4}$ & $4.02\rank{2}$ & $\winner{2.72}\rank{1}$ & $3.82\rank{2}$ \\%BPIC17
& Plaus &
 $9.11\rank{4}$ & $\winner{8.46}\rank{1}$ & $8.80\rank{4}$ & $\winner{8.83}\rank{1}$ & $\winner{8.70}\rank{1}$ &%SYNTH
 $7.86\rank{2}$ & $\winner{6.38}\rank{1}$ & $9.73\rank{3}$ & $9.67\rank{3}$ & $9.70\rank{3}$ &%BPIC2012
 $7.57\rank{5}$ & $7.39\rank{4}$ & $\winner{5.52}\rank{1}$ & $\winner{4.94}\rank{1}$ & $\winner{5.40}\rank{1}$ \\%BPIC17
& Conf &
 $0.71\rank{5}$ & $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
 $0.72\rank{5}$ & $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
 $0.86\rank{5}$ & $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dive &
 $0.47\rank{3}$ & $0.47\rank{3}$ & $0.50\rank{2}$ & $\winner{0.52}\rank{1}$ & $0.49\rank{3}$ &%SYNTH
 $\winner{0.40}\rank{1}$ & $0.36\rank{3}$ & $\winner{0.38}\rank{1}$ & $0.32\rank{5}$ & $0.35\rank{3}$ &%BPIC2012
 $\winner{0.61}\rank{1}$ & $\winner{0.60}\rank{1}$ & $0.34\rank{3}$ & $0.26\rank{5}$ & $0.33\rank{3}$ \\%BPIC17
& Run &
 $\winner{1.0}\rank{1}$ & $2.76\rank{2}$ & $4.41\rank{5}$ & $3.10\rank{2}$ & $3.23\rank{2}$ &%SYNTH
 $\winner{2.5}\rank{1}$ & $154\rank{2}$ & $211\rank{2}$ & $133\rank{2}$ & $191\rank{2}$ &%BPIC2012
 $\winner{5.4}\rank{1}$ & $29.1\rank{2}$ & $81.6\rank{4}$ & $54.4\rank{2}$ & $75.6\rank{4}$ \\%BPIC17
\midrule
\multirow{6}{*}{50\%} 
& Dist &
 $0.34\rank{4}$ & $0.41\rank{5}$ & $0.27\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.27\rank{2}$ &%SYNTH
 $0.46\rank{2}$ & $0.55\rank{5}$ & $0.20\rank{3}$ & $\winner{0.24}\rank{1}$ & $0.30\rank{2}$ &%BPIC2012
 $0.58\rank{4}$ & $0.6\rank{4}$ & $0.17\rank{2}$ & $\winner{0.09}\rank{1}$ & $0.18\rank{2}$ \\%BPIC17
& Spars &
 $1.82\rank{4}$ & $2.19\rank{5}$ & $1.41\rank{2}$ & $\winner{1.17}\rank{1}$ & $1.40\rank{2}$ &%SYNTH
 $6.69\rank{2}$ & $7.83\rank{5}$ & $5.55\rank{3}$ & $\winner{3.52}\rank{1}$ & $4.11\rank{2}$ &%BPIC2012
 $6.91\rank{4}$ & $7.11\rank{4}$ & $2.06\rank{2}$ & $\winner{1.06}\rank{1}$ & $2.16\rank{2}$ \\%BPIC17
& Impl. &
 $\winner{6.80}\rank{1}$ & $7.17\rank{3}$ & $7.17\rank{3}$ & $\winner{7.01}\rank{1}$ & $7.16\rank{3}$ &%SYNTH
 $8.12\rank{4}$ & $\winner{7.58}\rank{1}$ & $8.51\rank{4}$ & $\winner{7.28}\rank{1}$ & $\winner{7.13}\rank{1}$ &%BPIC2012
 $8.29\rank{4}$ & $7.95\rank{4}$ & $4.86\rank{2}$ & $\winner{4.38}\rank{1}$ & $5.14\rank{2}$ \\%BPIC17
& Conf &
 $0.67\rank{5}$ & $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
 $0.70\rank{5}$ & $\winner{0.97}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
 $0.80\rank{5}$ & $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dive &
 $0.38\rank{2}$ & $\winner{0.43}\rank{1}$ & $0.30\rank{3}$ & $0.25\rank{5}$ & $0.30\rank{3}$ &%SYNTH
 $\winner{0.41}\rank{1}$ & $\winner{0.36}\rank{1}$ & $0.19\rank{5}$ & $0.25\rank{3}$ & $0.27\rank{3}$ &%BPIC2012
 $\winner{0.63}\rank{1}$ & $\winner{0.61}\rank{1}$ & $0.18\rank{3}$ & $0.11\rank{5}$ & $0.19\rank{3}$ \\%BPIC17
& Run &
 $\winner{1.0}\rank{1}$ & $3.39\rank{2}$ & $9.78\rank{5}$ & $4.80\rank{3}$ & $5.18\rank{3}$ &%SYNTH
 $\winner{2.5}\rank{1}$ & $535\rank{3}$ & $1500\rank{5}$ & $451\rank{2}$ & $780\rank{3}$ &%BPIC2012
 $\winner{5.50\rank{1}}$ & $288\rank{2}$ & $566\rank{2}$ & $261\rank{2}$ & $463\rank{2}$ \\%BPIC17
\bottomrule
\end{tabular}}}
\caption{Performance metrics across different datasets. \massi{The ranking position of each method is indicated after the pipe $|$.}}
\label{tab:diffs}
\end{table*}


%%%%NEW TABLE
\begin{table*}[t]
\centering
{\fontsize{9pt}{10pt}\selectfont
\scalebox{0.75}{
\begin{tabular}{llcccc|cccc|cccc}
\toprule
\multirow{2}{*}{$\frac{|\tasks_\varphi|}{|\tasks|}$}  &  & \multicolumn{5}{c}{Claim Management} & \multicolumn{5}{c}{BPIC2012} &  \multicolumn{5}{c}{BPIC2017}  \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17}
 & & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort  & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur \\
\midrule
 \multirow{6}{*}{10\%} 
 Conf &
   $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
 & Dist &
  $0.48\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ &%SYNTH
 $\winner{0.47}\rank{1}$ & $0.54\rank{5}$ & $0.50\rank{2}$ & $\winner{0.47}\rank{1}$ & $0.50\rank{2}$ &%BPIC2012
 $0.58\rank{4}$ & $0.59\rank{4}$ & $0.50\rank{2}$ & $\winner{0.44}\rank{1}$ & $0.50\rank{2}$ \\ %BPIC17
& Spars &
   $2.50\rank{2}$ & $2.58\rank{2}$ & $2.63\rank{2}$ & $2.58\rank{2}$ &%SYNTH
   $7.69\rank{5}$ & $\winner{6.95}\rank{1}$ & $\winner{6.79}\rank{1}$ & $\winner{6.97}\rank{1}$ &%BPIC2012
   $6.95\rank{4}$ & $\winner{5.60}\rank{1}$ & $\winner{5.20}\rank{1}$ & $5.85\rank{3}$ \\%BPIC17
& Plaus &
   $\winner{8.49}\rank{1}$ & $8.88\rank{2}$ & $8.84\rank{2}$ & $8.92\rank{2}$ &%SYNTH
  $\winner{7.49}\rank{1}$ & $\winner{7.37}\rank{1}$ & $\winner{7.26}\rank{1}$ & $\winner{7.38}\rank{1}$ &%BPIC2012
  $\winner{7.51}\rank{1}$ & $\winner{6.81}\rank{1}$ & $\winner{6.59}\rank{1}$ & $\winner{6.86}\rank{1}$ \\%BPIC17
& Dive &
   $0.48\rank{4}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ &%SYNTH
   $0.35\rank{5}$ & $\winner{0.40}\rank{1}$ & $\winner{0.41}\rank{1}$ & $\winner{0.40}\rank{1}$ &%BPIC2012
   $0.58\rank{2}$ & $0.49\rank{3}$ & $0.44\rank{5}$ & $0.49\rank{3}$ \\ %BPIC17
 & Run &
  $2.53\rank{2}$ & $4.65\rank{5}$ & $4.38\rank{3}$ & $4.09\rank{3}$ &%SYNTH
   $25\rank{4}$ & $90\rank{5}$ & $12\rank{2}$ & $17\rank{3}$ &%BPIC2012
   $29.1\rank{2}$ & $78.3\rank{3}$ & $57.3\rank{3}$ & $65.5\rank{3}$ \\%BPIC17
\midrule
\multirow{6}{*}{25\%} 
 Conf &
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dist &
   $0.48\rank{2}$ & $0.47\rank{2}$ & $0.50\rank{5}$ & $0.47\rank{2}$ &%SYNTH
   $0.47\rank{2}$ & $0.38\rank{4}$ & $\winner{0.30}\rank{1}$ & $0.36\rank{2}$ &%BPIC2012
  $0.58\rank{4}$ & $0.33\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.31\rank{2}$ \\%BPIC17
& Spars &
   $2.50\rank{2}$ & $2.45\rank{2}$ & $2.58\rank{5}$ & $2.42\rank{2}$ &%SYNTH
   $7.01\rank{3}$ & $5.24\rank{3}$ & $\winner{4.38}\rank{1}$ & $4.92\rank{2}$ &%BPIC2012
   $6.77\rank{4}$ & $4.02\rank{2}$ & $\winner{2.72}\rank{1}$ & $3.82\rank{2}$ \\%BPIC17
& Plaus &
   $\winner{8.46}\rank{1}$ & $8.80\rank{4}$ & $\winner{8.83}\rank{1}$ & $\winner{8.70}\rank{1}$ &%SYNTH
   $\winner{6.38}\rank{1}$ & $9.73\rank{3}$ & $9.67\rank{3}$ & $9.70\rank{3}$ &%BPIC2012
   $7.39\rank{4}$ & $\winner{5.52}\rank{1}$ & $\winner{4.94}\rank{1}$ & $\winner{5.40}\rank{1}$ \\%BPIC17
& Dive &
   $0.47\rank{3}$ & $0.50\rank{2}$ & $\winner{0.52}\rank{1}$ & $0.49\rank{3}$ &%SYNTH
   $0.36\rank{3}$ & $\winner{0.38}\rank{1}$ & $0.32\rank{5}$ & $0.35\rank{3}$ &%BPIC2012
  $\winner{0.60}\rank{1}$ & $0.34\rank{3}$ & $0.26\rank{5}$ & $0.33\rank{3}$ \\%BPIC17
& Run &
   $2.76\rank{2}$ & $4.41\rank{5}$ & $3.10\rank{2}$ & $3.23\rank{2}$ &%SYNTH
   $154\rank{2}$ & $211\rank{2}$ & $133\rank{2}$ & $191\rank{2}$ &%BPIC2012
   $29.1\rank{2}$ & $81.6\rank{4}$ & $54.4\rank{2}$ & $75.6\rank{4}$ \\%BPIC17
\midrule
\multirow{6}{*}{50\%} 
Conf &
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{0.97}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dist &
   $0.41\rank{5}$ & $0.27\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.27\rank{2}$ &%SYNTH
   $0.55\rank{5}$ & $0.20\rank{3}$ & $\winner{0.24}\rank{1}$ & $0.30\rank{2}$ &%BPIC2012
   $0.6\rank{4}$ & $0.17\rank{2}$ & $\winner{0.09}\rank{1}$ & $0.18\rank{2}$ \\%BPIC17
& Spars &
   $2.19\rank{5}$ & $1.41\rank{2}$ & $\winner{1.17}\rank{1}$ & $1.40\rank{2}$ &%SYNTH
   $7.83\rank{5}$ & $5.55\rank{3}$ & $\winner{3.52}\rank{1}$ & $4.11\rank{2}$ &%BPIC2012
  $7.11\rank{4}$ & $2.06\rank{2}$ & $\winner{1.06}\rank{1}$ & $2.16\rank{2}$ \\%BPIC17
& Impl. &
   $7.17\rank{3}$ & $7.17\rank{3}$ & $\winner{7.01}\rank{1}$ & $7.16\rank{3}$ &%SYNTH
   $\winner{7.58}\rank{1}$ & $8.51\rank{4}$ & $\winner{7.28}\rank{1}$ & $\winner{7.13}\rank{1}$ &%BPIC2012
   $7.95\rank{4}$ & $4.86\rank{2}$ & $\winner{4.38}\rank{1}$ & $5.14\rank{2}$ \\%BPIC17
& Dive &
   $\winner{0.43}\rank{1}$ & $0.30\rank{3}$ & $0.25\rank{5}$ & $0.30\rank{3}$ &%SYNTH
   $\winner{0.36}\rank{1}$ & $0.19\rank{5}$ & $0.25\rank{3}$ & $0.27\rank{3}$ &%BPIC2012
   $\winner{0.61}\rank{1}$ & $0.18\rank{3}$ & $0.11\rank{5}$ & $0.19\rank{3}$ \\%BPIC17
& Run &
   $3.39\rank{2}$ & $9.78\rank{5}$ & $4.80\rank{3}$ & $5.18\rank{3}$ &%SYNTH
   $535\rank{3}$ & $1500\rank{5}$ & $451\rank{2}$ & $780\rank{3}$ &%BPIC2012
   $288\rank{2}$ & $566\rank{2}$ & $261\rank{2}$ & $463\rank{2}$ \\%BPIC17
\bottomrule
\end{tabular}}}
\caption{Performance metrics across different datasets. \massi{The ranking position of each method is indicated after the pipe $|$.}}
\label{tab:diffs}
\end{table*}

==> new_results.tex <==
\section{Results}
\label{sec:results}


\begin{table*}[t]
\centering
{\fontsize{9pt}{10pt}\selectfont
\scalebox{0.75}{
\begin{tabular}{llcccc|cccc|cccc}
\toprule
\multirow{2}{*}{$\frac{|\tasks_\varphi|}{|\tasks|}$}  &  & \multicolumn{5}{c}{Claim Management} & \multicolumn{5}{c}{BPIC2012} &  \multicolumn{5}{c}{BPIC2017}  \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17}
 & & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort  & \marshort & \firstheur & \secondheur & \geneticshort & \ltlfbaseshort & \marshort & \firstheur & \secondheur \\
\midrule
 \multirow{6}{*}{10\%} 
 Conf &
   $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
 & Dist &
  $0.48\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ & $0.50\rank{2}$ &%SYNTH
 $\winner{0.47}\rank{1}$ & $0.54\rank{5}$ & $0.50\rank{2}$ & $\winner{0.47}\rank{1}$ & $0.50\rank{2}$ &%BPIC2012
 $0.58\rank{4}$ & $0.59\rank{4}$ & $0.50\rank{2}$ & $\winner{0.44}\rank{1}$ & $0.50\rank{2}$ \\ %BPIC17
& Spars &
   $2.50\rank{2}$ & $2.58\rank{2}$ & $2.63\rank{2}$ & $2.58\rank{2}$ &%SYNTH
   $7.69\rank{5}$ & $\winner{6.95}\rank{1}$ & $\winner{6.79}\rank{1}$ & $\winner{6.97}\rank{1}$ &%BPIC2012
   $6.95\rank{4}$ & $\winner{5.60}\rank{1}$ & $\winner{5.20}\rank{1}$ & $5.85\rank{3}$ \\%BPIC17
& Plaus &
   $\winner{8.49}\rank{1}$ & $8.88\rank{2}$ & $8.84\rank{2}$ & $8.92\rank{2}$ &%SYNTH
  $\winner{7.49}\rank{1}$ & $\winner{7.37}\rank{1}$ & $\winner{7.26}\rank{1}$ & $\winner{7.38}\rank{1}$ &%BPIC2012
  $\winner{7.51}\rank{1}$ & $\winner{6.81}\rank{1}$ & $\winner{6.59}\rank{1}$ & $\winner{6.86}\rank{1}$ \\%BPIC17
& Dive &
   $0.48\rank{4}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ & $\winner{0.54}\rank{1}$ &%SYNTH
   $0.35\rank{5}$ & $\winner{0.40}\rank{1}$ & $\winner{0.41}\rank{1}$ & $\winner{0.40}\rank{1}$ &%BPIC2012
   $0.58\rank{2}$ & $0.49\rank{3}$ & $0.44\rank{5}$ & $0.49\rank{3}$ \\ %BPIC17
 & Run &
  $2.53\rank{2}$ & $4.65\rank{5}$ & $4.38\rank{3}$ & $4.09\rank{3}$ &%SYNTH
   $25\rank{4}$ & $90\rank{5}$ & $12\rank{2}$ & $17\rank{3}$ &%BPIC2012
   $29.1\rank{2}$ & $78.3\rank{3}$ & $57.3\rank{3}$ & $65.5\rank{3}$ \\%BPIC17
\midrule
\multirow{6}{*}{25\%} 
 Conf &
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dist &
   $0.48\rank{2}$ & $0.47\rank{2}$ & $0.50\rank{5}$ & $0.47\rank{2}$ &%SYNTH
   $0.47\rank{2}$ & $0.38\rank{4}$ & $\winner{0.30}\rank{1}$ & $0.36\rank{2}$ &%BPIC2012
  $0.58\rank{4}$ & $0.33\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.31\rank{2}$ \\%BPIC17
& Spars &
   $2.50\rank{2}$ & $2.45\rank{2}$ & $2.58\rank{5}$ & $2.42\rank{2}$ &%SYNTH
   $7.01\rank{3}$ & $5.24\rank{3}$ & $\winner{4.38}\rank{1}$ & $4.92\rank{2}$ &%BPIC2012
   $6.77\rank{4}$ & $4.02\rank{2}$ & $\winner{2.72}\rank{1}$ & $3.82\rank{2}$ \\%BPIC17
& Plaus &
   $\winner{8.46}\rank{1}$ & $8.80\rank{4}$ & $\winner{8.83}\rank{1}$ & $\winner{8.70}\rank{1}$ &%SYNTH
   $\winner{6.38}\rank{1}$ & $9.73\rank{3}$ & $9.67\rank{3}$ & $9.70\rank{3}$ &%BPIC2012
   $7.39\rank{4}$ & $\winner{5.52}\rank{1}$ & $\winner{4.94}\rank{1}$ & $\winner{5.40}\rank{1}$ \\%BPIC17
& Dive &
   $0.47\rank{3}$ & $0.50\rank{2}$ & $\winner{0.52}\rank{1}$ & $0.49\rank{3}$ &%SYNTH
   $0.36\rank{3}$ & $\winner{0.38}\rank{1}$ & $0.32\rank{5}$ & $0.35\rank{3}$ &%BPIC2012
  $\winner{0.60}\rank{1}$ & $0.34\rank{3}$ & $0.26\rank{5}$ & $0.33\rank{3}$ \\%BPIC17
& Run &
   $2.76\rank{2}$ & $4.41\rank{5}$ & $3.10\rank{2}$ & $3.23\rank{2}$ &%SYNTH
   $154\rank{2}$ & $211\rank{2}$ & $133\rank{2}$ & $191\rank{2}$ &%BPIC2012
   $29.1\rank{2}$ & $81.6\rank{4}$ & $54.4\rank{2}$ & $75.6\rank{4}$ \\%BPIC17
\midrule
\multirow{6}{*}{50\%} 
Conf &
   $\winner{0.99}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%SYNTH
   $\winner{0.97}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ &%BPIC2012
   $\winner{0.98}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ & $\winner{1.0}\rank{1}$ \\%BPIC17
& Dist &
   $0.41\rank{5}$ & $0.27\rank{2}$ & $\winner{0.22}\rank{1}$ & $0.27\rank{2}$ &%SYNTH
   $0.55\rank{5}$ & $0.20\rank{3}$ & $\winner{0.24}\rank{1}$ & $0.30\rank{2}$ &%BPIC2012
   $0.6\rank{4}$ & $0.17\rank{2}$ & $\winner{0.09}\rank{1}$ & $0.18\rank{2}$ \\%BPIC17
& Spars &
   $2.19\rank{5}$ & $1.41\rank{2}$ & $\winner{1.17}\rank{1}$ & $1.40\rank{2}$ &%SYNTH
   $7.83\rank{5}$ & $5.55\rank{3}$ & $\winner{3.52}\rank{1}$ & $4.11\rank{2}$ &%BPIC2012
  $7.11\rank{4}$ & $2.06\rank{2}$ & $\winner{1.06}\rank{1}$ & $2.16\rank{2}$ \\%BPIC17
& Impl. &
   $7.17\rank{3}$ & $7.17\rank{3}$ & $\winner{7.01}\rank{1}$ & $7.16\rank{3}$ &%SYNTH
   $\winner{7.58}\rank{1}$ & $8.51\rank{4}$ & $\winner{7.28}\rank{1}$ & $\winner{7.13}\rank{1}$ &%BPIC2012
   $7.95\rank{4}$ & $4.86\rank{2}$ & $\winner{4.38}\rank{1}$ & $5.14\rank{2}$ \\%BPIC17
& Dive &
   $\winner{0.43}\rank{1}$ & $0.30\rank{3}$ & $0.25\rank{5}$ & $0.30\rank{3}$ &%SYNTH
   $\winner{0.36}\rank{1}$ & $0.19\rank{5}$ & $0.25\rank{3}$ & $0.27\rank{3}$ &%BPIC2012
   $\winner{0.61}\rank{1}$ & $0.18\rank{3}$ & $0.11\rank{5}$ & $0.19\rank{3}$ \\%BPIC17
& Run &
   $3.39\rank{2}$ & $9.78\rank{5}$ & $4.80\rank{3}$ & $5.18\rank{3}$ &%SYNTH
   $535\rank{3}$ & $1500\rank{5}$ & $451\rank{2}$ & $780\rank{3}$ &%BPIC2012
   $288\rank{2}$ & $566\rank{2}$ & $261\rank{2}$ & $463\rank{2}$ \\%BPIC17
\bottomrule
\end{tabular}}}
\caption{Performance metrics across different datasets. \massi{The ranking position of each method is indicated after the pipe $|$.}}
\label{tab:diffs}
\end{table*}



To analyse the results, Table~\ref{tab:diffs} shows the average values of each method, together with its afferent rank \rtext{(in parentheses)} to show statistically significant differences between the methods for each evaluation metric. We show the evolution of the results with varying levels of coverage $|\tasks_\varphi|/|\tasks|$.


\textbf{Answering RQ1:} 
In the Claim Management dataset, differences between methods are less pronounced but still noticeable across various metrics. For \dist and \spars, \geneticshort yields the closest counterfactuals at 10\% and 25\% coverage, while \firstheur and \secondheur perform better at 50\% for both \dist and \spars. Regarding \impl, all methods exhibit similar performance; however, \ltlfbaseshort and the proposed methods slightly outperform \geneticshort and \marshort, particularly at higher coverage levels (25\%,50\%). For conformance, \geneticshort consistently performs the worst, with the proposed methods,~\marshort maintaining full adherence to the temporal constraints. For larger coverage, \ltlfbaseshort does not maintain the full adherence to the constraints. In \dive, \marshort produces the most diverse counterfactuals at all coverage levels, with \geneticshort also showing high diversity. The proposed methods generate less diverse counterfactuals, particularly at 50\% coverage.
For \dive, for lower coverage (10\%, 25\%) \firstheur produces the most diverse counterfactuals, with \mar and \secondheur slightly below, while the other two baselines performing worse. For 50\% however, \ltlfbaseshort performs best, with \firstheur performing worst. 
Lastly, for \run, \geneticshort achieves the shortest runtime across all coverage levels, followed by \ltlfbaseshort. \firstheur and \secondheur have a higher \run than \geneticshort and \ltlfbaseshort, although \marshort has a higher \run, especially at higher coverages.

Regarding BPIC2012, the performance of the proposed  and baseline approaches tends to vary across the metrics. For distance, at 10\% coverage, \firstheur and \secondheur surpass the baselines, with \secondheur performing comparably to \geneticshort and closely trailing \firstheur. At higher coverage levels, \firstheur outperforms all other methods, yielding the closest counterfactuals, whereas \ltlfbaseshort generates the most distant examples. Regarding \spars, all methods show similar levels at 10\% coverage, with \ltlfbaseshort producing slightly less sparse counterfactuals. As coverage increases, the proposed methods (\firstheur and \secondheur) retain superior performance, with \firstheur consistently providing the sparsest counterfactuals and significantly outperforming \ltlfbaseshort and \geneticshort. In terms of \impl, \ltlfbaseshort performs best across all coverage levels, while \marshort tends to produce less plausible counterfactuals. The proposed methods rank similarly to \geneticshort and outperform \marshort, particularly at higher coverage levels. For conformance, \ltlfbaseshort demonstrates high adherence to the temporal background knowledge across all coverage levels, marginally outperforming the proposed methods, which still perform better than \geneticshort, indicating its higher tendency to violate temporal constraints. In diversity, the proposed methods, notably \secondheur, produce less diverse counterfactuals at all coverage levels, with \marshort and \geneticshort showing the highest diversity. As coverage increases, the diversity gap between the proposed methods and baselines like \geneticshort widens. Lastly, for \run, \geneticshort has the shortest \run at all coverage levels, followed by \ltlfbaseshort. \firstheur and \secondheur have a higher \run, with \secondheur increasing with higher coverage levels, while \marshort consistently shows the highest \run.


For BPIC2017, performance varies notably with coverage levels. For \dist and \spars, \firstheur excels at all coverage levels, producing the closest counterfactuals, with \secondheur and \marshort following but remaining slightly behind, especially at 50\% coverage where \geneticshort and \ltlfbaseshort yield more distant results. Regarding \impl, \firstheur and \ltlfbaseshort deliver the most plausible counterfactuals consistently, outshining \geneticshort and \secondheur, with \marshort producing the least plausible results, though improving at 50\% coverage. For conformance, \firstheur, \secondheur, and \ltlfbaseshort show high adherence to temporal constraints, while \geneticshort has a low \sat, particularly at lower coverage levels. \dive is highest for the proposed methods at 10\% coverage, although performing worse w.r.t all baseline methods, but this advantage diminishes as coverage increases, with \firstheur and \secondheur demonstrating lower diversity at 25\% and 50\% coverage. Finally, in terms of \run, \geneticshort and \ltlfbaseshort are the best, while the proposed methods, especially \secondheur, require more time, with \marshort showing the longest runtime, particularly for higher coverage.

Overall, the proposed methods demonstrate superior performance in \sat, \spars, and \dist across both datasets, although they tend to produce less diverse counterfactuals and require more runtime compared to baselines like \geneticshort and \ltlfbaseshort. These results emphasize the trade-offs between different evaluation metrics depending on the coverage level, with the proposed strategies showing their strengths particularly in scenarios where preserving the temporal background knowledge is crucial.
%Overall, we observe some general trends across all datasets: the proposed methods can produce on average closer, more sparse, but also less diverse and require longer to generate the desired counterfactuals, whilst guaranteeing the satisfaction of the provided temporal background knowledge. Thus, if diversity is a critical desideratum, and the generated examples are not required to satisfy the background knowledge, the baseline method \genetic is desired. If, however, conformance becomes more important as a desideratum, although not strictly necessary, \ltlfbase can be used to decrease the trade-off in diversity. In more critical applications domains, however, only the proposed methods \firstheur and \secondheur can preserve the given background knowledge, while all other methods cannot guarantee it.~\mar requires the longest amount of runtime, without however providing a significant difference over the other methods, either in terms of diversity or distance.

\textbf{Answering RQ2:} For the Claim Management dataset, with a coverage of 10\%, both methods perform similarly, with both methods register equally higher counterfactual quality measures, with no significant difference. For larger coverages, the results change: for 25\%, \firstheur produces the least sparse and most distant counterfactuals, although also the most diverse ones, while \secondheur performs better for \spars and \dist, although with a lower \dive level. This behaviour thoroughly changes for 50\% coverage, where \firstheur performs the best for \dist, \spars, and \impl, while \secondheur outperforms in \dive.
In the BPIC2012 dataset, while for lower coverage (10\%), the two methods perform similarly, for increasing coverage levels, \firstheur excels in producing closer and more sparse counterfactuals compared to \secondheur, but \secondheur achieves greater diversity, although with no significant difference for 50\% coverage. Additionally, there is a significant difference in runtime between the two methods, with \firstheur generally being faster, especially as coverage increases.
For the BPIC2017 dataset, \firstheur typically generates counterfactuals that are closer, and more sparse. However, this advantage comes with a trade-off in diversity, where \firstheur produces less diverse counterfactuals. In contrast, \secondheur strikes a better balance between distance, sparsity, \impl, and diversity, although requiring a longer runtime. The impact of these trade-offs becomes more pronounced with the increasing complexity of the formula.

Overall, while \firstheur offers advantages in terms of \dist, \spars, and sometimes \impl,~\secondheur may provide a better trade-off between these metrics and \dive. The choice of strategy depends on whether the priority is to maximize \dist and \spars or to enhance \dive, though these benefits come at the expense of higher \run, particularly with more complex $\varphi$, i.e.~greater size of $\tasks_\varphi$.

%\subsection{Discussion}
%We concluded the analysis of the results saying the choice between the strategy to use depends upon the size of $\tasks_\vaprhi$,as the number of activities in this set may have an influence on the resulting $\varphi$ and its corresponding \DFA. This in turn has an effect on the amount of time required to check the \sat of each individual member of the population, which is especially evident for \mar, where after each mutation attempt, we perform a check on the compliance of the counterfactual candidate. Thus, as observed in Table~\ref{tab:diffs}, we observe that, for each dataset used, as coverage increases, we see a significant increase between the differences of all methods when compared to \mar. A potential way to overcome this issue is to try different reasoners

%Overall, as coverage levels increase from 10\% to 50\%, there are notable shifts in the average results of various metrics. Distance between generated counterfactuals and the original instances typically increases, reflecting the growing challenge of maintaining proximity as more attributes are covered. Sparsity tends to decrease with higher coverage; counterfactuals become less sparse as they need to address a broader range of attributes. \impl shows a moderate improvement or stabilization, as counterfactuals at higher coverage levels generally conform better to the data distribution, assuming that other metrics do not significantly compromise it. Conformance remains consistently high across coverage levels, indicating robust adherence to temporal constraints. Diversity of counterfactuals increases with coverage, as more attributes lead to a broader range of possible counterfactuals. However, this comes at the cost of increased runtime, which grows significantly as the complexity of covering more attributes expands. Overall, while higher coverage enhances diversity and complexity, it also demands greater computational resources and tends to reduce the closeness and sparsity of counterfactuals.
%The metric with the highest influence from the coverage levels tends to be \run, as the \DFA corresponding to the specific $\varphi$ formula may require more and more time to check each generated trace. Moreover, as can be observed from Table~\ref{tab:dataset}, we observe larger increases in runtime for dataset where we have traces with longer average prefix lengths.

==> old_intro.tex <==
\section{Introduction}

State-of-the-art efforts in Machine Learning have focused on delivering accurate predictive models through the application of ensemble learning and deep learning techniques. Due to the inherent complexity of these models, commonly referred to as \emph{black-box} models, they are often challenging for users to comprehend. For this reason, eXplainable Artificial Intelligence (XAI) techniques have been recently adopted to help interpret their predictions and foster adoption of these advanced predictive models~\cite{verma2020counterfactual,guidotti2022counterfactual,moc,priorxai}.%

One example of such XAI techniques are counterfactual explanations, which suggest what should be different in the input instance to change the outcome of a prediction returned by a black-box predictive model. Most state-of-the-art counterfactual generation techniques in XAI are based around optimisation techniques~\cite{guidotti2022counterfactual}. Such techniques find the minimum change to the input that flips the prediction. 
Counterfactual explanations are essential for providing alternatives to achieve a certain outcome (\emph{outcome-based predictions}). They can guide users in modifying their input to reach a desired outcome by assisting them in understanding how various attributes may affect the input's outcome.
Most counterfactual explanation generation techniques, however, cannot account for the dependencies within temporal data typically represented by finite sequences $( e_1, e_2, \dots, e_n)$ of events $e_i$ such that each $e_i$ happens before $e_{i+1}$. Such sequences of data, often called \emph{event traces}, can represent e.g., the events happening to a patient in a surgery room, or in a clinical pathway, the events one performs to accomplish a certain administrative procedure, business matter, or even the events that a certain object undergoes to in an assembly line.   
This data is increasingly used to train predictive models for outcome-based predictions and would thus benefit from generating counterfactual explanations.  
Moreover, little effort has been given to constraining counterfactual explanations through background knowledge, especially in terms of temporal background knowledge. This is an important problem to address, since the e.g.,  medical, administrative, business, or industrial domains mentioned above often include constraints that reflect the actual domain and that must be adhered to when generating counterfactuals.   
%As an example, suppose that a counterfactual suggests to a customer that a loan application submission has to be performed before the loan application is actually filled in, in order to change the prediction from rejected to accepted. This scenario would not benefit the expert trying to explain the predictive model nor a hypothetic customer using the counterfactual to have the loan accepted. In fact, the counterfactual is infeasible, as it goes against the logical sequence of events.

To fill the previously mentioned gap, in this work, we propose a novel counterfactual generation approach for temporal data in the form of event traces. Moreover, the method considers \LTLf formulae as temporal background knowledge to ensure the generation of counterfactual explanations that satisfy the given formulae.
From a technical standpoint, this is performed by adapting a Genetic Algorithm (GA)-based method to incorporate this temporal background knowledge by leveraging their standard characterisation based on deterministic finite-state automata (DFA). In particular, we adapt a GA's fitness function, as well as the crossover and mutation operators, to incorporate a set of \LTLf formulae, represented through their conjunction, and their standard characterisation based on DFA.
Since the combination between the Genetic Algorithm and the deterministic finite-state automata can be done in different ways, in this paper we explore three different strategies that incorporate this \LTLf-based temporal background knowledge: one strategy works in an \emph{a priori} fashion, extracting the information required from the DFA beforehand, while two other strategies focus on traversing the extracted DFA to guide the GA at runtime in an \emph{online} fashion, thus avoiding any violations of the given temporal background knowledge. 
In this way, we aim to generate counterfactuals that satisfy the formulae, whilst maintaining general counterfactual desiderata.

An empirical evaluation on real-world and synthetic datasets confirms the effectiveness of our approach, with respect to using only state of the art GAs. 
The results suggest that the proposed approaches that include the temporal background knowledge can produce better counterfactuals explanations, especially in satisfying the \LTLf formulae, whilst maintaining or improving counterfactual desiderata.

Therefore, this work enhances model interpretability by aligning counterfactuals with temporal background knowledge, thereby improving the practical utility of ``black-box'' predictive models.
 
The paper is structured as follows. Section~\ref{sec:background} introduces the main background concepts, Section~\ref{sec:relwork} discusses related work, Section~\ref{sec:approach} highlights the contributions of this work, while Section~\ref{sec:eval} introduces the evaluation and experimental settings. The results are reported 
in Section~\ref{sec:results}, while the conclusions are outlined
in Section~\ref{sec:conclusions}.

==> old_results.tex <==
\section{Results}
\label{sec:results}

%\begin{figure*}[h!]
%    \centering
%    \includegraphics[width=\textwidth,height=4.8cm]{plots/merged_plots_final.png}
%    \caption{Overall evaluation results for the Claim Management and BPIC2012 datasets}
%    \label{fig:overallboxplots}
%\end{figure*}

\begin{table*}[t]
\centering
{\fontsize{9pt}{9pt}\selectfont
\begin{tabular}{ccccccc|ccccc|ccccc}
\toprule
Cov. & Metric & \multicolumn{5}{c}{BPIC17} & \multicolumn{5}{c}{BPIC2012} & \multicolumn{5}{c}{Synthetic Data} \\ \midrule
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17}
 & & Gen & $Gen_\varphi$ & H1 & H2 & MAR & Gen & $Gen_\varphi$ & H1 & H2 & MAR & Gen & $Gen_\varphi$ & H1 & H2 & MAR \\
\midrule
 \multirow{6}{*}{10\%} & Conf & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 \\
 & Dist & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
 & Dive & 4 & 4 & 1 & 2 & 2 & 4 & 1 & 1 & 2 & 3 & 1 & 2 & 1 & 1 & 1 \\
 & Impl & 4 & 4 & 1 & 2 & 2 & 2 & 1 & 1 & 1 & 2 & 2 & 2 & 2 & 2 & 2 \\
 & Run & 1 & 2 & 3 & 4 & 4 & 1 & 3 & 2 & 3 & 5 & 1 & 2 & 3 & 3 & 5 \\
 & Spars & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
 \midrule
 \multirow{6}{*}{25\%} & Conf & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 \\
 & Dist & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
 & Dive & 4 & 4 & 1 & 2 & 2 & 4 & 1 & 1 & 2 & 3 & 1 & 2 & 1 & 1 & 1 \\
 & Impl & 4 & 4 & 1 & 2 & 2 & 2 & 1 & 1 & 1 & 2 & 2 & 2 & 2 & 2 & 2 \\
 & Run & 1 & 2 & 3 & 4 & 4 & 1 & 3 & 2 & 3 & 5 & 1 & 2 & 3 & 3 & 5 \\
 & Spars & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
 \midrule
 \multirow{6}{*}{50\%} & Conf & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 & 1 & 2 & 2 & 2 & 2 \\
 & Dist & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
 & Dive & 4 & 4 & 1 & 2 & 2 & 4 & 1 & 1 & 2 & 3 & 1 & 2 & 1 & 1 & 1 \\
 & Impl & 4 & 4 & 1 & 2 & 2 & 2 & 1 & 1 & 1 & 2 & 2 & 2 & 2 & 2 & 2 \\
 & Run & 1 & 2 & 3 & 4 & 4 & 1 & 3 & 2 & 3 & 5 & 1 & 2 & 3 & 3 & 5 \\
 & Spars & 4 & 4 & 1 & 2 & 2 & 2 & 5 & 1 & 2 & 3 & 1 & 4 & 1 & 1 & 1 \\
\bottomrule
\end{tabular}}
\caption{Performance metrics across different datasets and coverage levels, including sparsity and excluding hit rate.}
\label{tab:diffs}
\end{table*}


In this section, we present %aim at presenting 
the results of the experiments to answer the research questions introduced in Section~\ref{sec:eval}.
%
Table~\ref{tab:diffs} illustrates the evaluation results for both the %synthetic 
Claim Management and the BPIC2012 datasets. We first compare the two proposed strategies against the three baseline methods %: 
i.e., \genetic, and \ltlfbase, and \mar, %.
%We first highlight the overall differences between baselines and proposed strategies 
so as to address \textbf{\ref{RQ1};} we then proceed to tackle \textbf{\ref{RQ2}} by comparing the results of %among 
the two proposed strategies. %Finally, \ref{RQ3} will be addressed by observing how alphabet size $\Sigma$ relative to the entire alphabet $\mathcal{V}$, that is used to build $\varphi$, influences the generated counterfactual explanations' outcomes.
Finally, we address \textbf{\ref{RQ3}} by observing how the percentage of 
 the alphabet $|\Sigma|/|\mathcal{V}|$ used to build $\varphi$ influences the generated counterfactuals' outcomes.

\textbf{Answering \ref{RQ1}.}
In Table~\ref{tab:diffs}, we see that
all proposed strategies produce counterfactuals closer to the input instance, i.e., lower \dist and %less 
\spars with respect to the baselines. Indeed, they all make 
%, making 
less changes to the input instance to generate the counterfactuals, especially as %we increase 
the coverage of $\Sigma$ over $\mathcal{V}$ increases. In terms of \impl, there are no significant differences between the baselines and the proposed strategies. Focusing on the \sat, %Moreover, 
we observe that the proposed strategies generate counterfactuals always satisfying the \LTLf %given 
formula, differently from %while 
the 
baseline methods that %\genetic and \ltlfbase 
show violations of the given temporal background knowledge. Although %While 
\ltlfbase has %registers 
a higher \sat than \genetic, the method can not %does not 
guarantee that the given formula $\varphi$ will be satisfied.
For \dive, the proposed strategies register comparable results, although the results depend upon the $\varphi$ that is used, as a  larger $\Sigma$ leads to a decrease in \dive for the proposed strategies, as a larger portion of the input instance is constrained.
In terms of \run, the proposed strategies require more time to generate the counterfactuals, although in some cases (when $\varphi$ only contains a 10\% of the alphabet for both datasets), %(the 10\% coverage for both datasets), 
the proposed strategies obtain %register 
comparable results. 

Overall, all the proposed methods generate counterfactuals with lower \dist and \spars, %less \dist, less \spars, 
that maximize \sat, while having a trade-off in terms of the \dive of the generated counterfactuals when compared to the baseline methods. While more diverse, counterfactuals generated with the baseline methods have the risk of violating $\varphi$, especially for the \genetic method. Moreover, the differences in \dive depend upon the choice of $\Sigma$ and $\varphi$ used: while smaller %. Smaller 
sizes of $\Sigma$ yield very similar results, for larger sizes the baseline methods produce more diverse counterfactuals.
%; however, the proposed strategies have a \sat of 100\%.
%Between the baselines, \ltlfbase provides a good trade-off between the \dive of the counterfactuals, their \sat, and \run, producing more diverse counterfactuals than \genetic, while having a higher \sat and only a slight increase in terms of \run. 


\textbf{Answering \ref{RQ2}.}
When looking at Table.~\ref{tab:diffs}, general differences can be observed among %between 
the three proposed strategies. Firstly, the \emph{a priori} strategy \firstheur produces counterfactuals, with overall the lowest \dist among %between 
all the strategies. Conversely, the online strategy, \secondheur, tends to yield counterfactuals with a higher \dist score.
Moreover, across various experimental settings, no considerable differences can be observed in terms of \spars and \impl.
%all methods demonstrate a tendency to produce counterfactuals with \cdf{lower} %less 
%\spars, i.e., \cdf{a} smaller number of changed attributes, with no large differences between the strategies. 
%Notably, for \impl, all strategies exhibit similar performance, indicating a consistent approach across different scenarios in generating counterfactuals that resemble the original data.
All proposed strategies achieve a notable 100\% in terms of \sat and \hr. 
%, as they always generate counterfactual explanations that satisfy $\varphi$.
Regarding \dive, the two \emph{online} strategies stand out for producing counterfactuals with a higher overall \dive, with \mar producing the most diverse counterfactuals, closely followed by \secondheur. Conversely, the \emph{a priori} strategy, \firstheur tends to yield counterfactuals with a lower \dive. 
Regarding \run, %the \emph{a priori} 
\firstheur generally requires less time to generate the counterfactuals, while %the \emph{online} methods 
\secondheur and \mar register a higher \run. Overall, \mar presents %registers 
the highest %overall 
variations for \run, depending on the number of times the mutation operation has to be repeated. %since the strategy may require to repeat re-doing the mutation operator.
%
%Moreover, the results can vary greatly depending upon the underlying DFA that is fed into the GA, as the method is dependent upon the structure of the automaton.
As expected, %between all three proposed strategies, the \thirdheur generated 
\mar generates the counterfactuals with the highest \dive, that always satisfies $\varphi$. Since \mar does not directly impose constraints on the mutation operator, it offers a greater flexibility. If a sampled action would violate $\varphi$, this method can resample and choose an alternative action to avoid the violation.
In general, while \mar produces the results with the highest %most 
\dive, it is also the strategy with the highest %most 
variability, especially in terms of other metrics such as \dist and \spars, and \run, while \secondheur provides the best trade-off in terms of all the metrics. 

In summary, the proposed methods offer different trade-offs, depending on which desiderata are most important for the user.
%Overall, the proposed methods offer different trade-offs, as they depend upon which desiderata are the most important for the user.
For more \emph{diverse} counterfactuals that satisfy $\varphi$, the \mar strategy offers the best overall \dive. 
If instead, \dist and \spars are important for the user, the \secondheur strategy offers \emph{closer} and more \emph{sparse} (i.e., with a lower number of attributes changed) %least changed attributes) 
counterfactuals, while maintaining a high level of \dive. Finally, \firstheur offers a lower \run together with lower \dist and \spars, %and coupled with more \emph{close} and \emph{sparse} counterfactuals, 
at the expense of a lower \dive.

\textbf{Answering \ref{RQ3}.}
In Table~\ref{tab:diffs}, the left part displays results for the Claim Management dataset, while on the right we have the results for the BPIC2012 dataset. Each row corresponds to an experiment using different levels of coverage, as mentioned in Sec.~\ref{sec:eval}. %Here, formulas cover $10\% (4 \text{ variables})$, $25\% (8 \text{ variables})$, and $50\% (16 \text{ variables})$ of $\mathcal{V}$.
We note that BPIC2012 has a larger set of variables for each experiment, leading to significant differences in runtime compared to the Claim Management dataset. Additionally, the average trace length in BPIC2012 is twice that %double that 
of the Claim Management dataset.

Overall, as alphabet coverage increases, differences between proposed methods and baselines also increase, particularly in terms of \dist, \spars, \dive, and \sat. Specifically, at 10\% coverage, little variation is observed in \dist, \spars, and \dive for proposed methods. %For both datasets, as \cdf{the} alphabet coverage rises, disparities between baselines and proposed \cdf{strategies} %methods 
%widen. %As expected, with increased coverage, the \dive of proposed methods decreases, albeit accompanied by lower \dist and \spars levels compared to baselines, which are less affected by coverage due to absence of constraints during counterfactual generation. 
As expected, an increase in coverage leads to a decrease in the \dive of the proposed strategies, coupled however with a decrease in \dist and \spars compared to the baselines.
%. However, this decrease comes together with a lower \dist and \spars 
%compared to the baselines.
On the contrary, the baselines are less affected by coverage variations because of the absence of constraints in the 
counterfactual generation.
%Moreover, as the GA's choices become more restricted, baseline methods, especially \genetic, exhibit more violations of $\varphi$, while \ltlfbase shows improvement with larger formulas, attributed to its use of $o_5$ facilitating faster convergence and higher \sat.
Moreover, as the coverage increases, baseline methods, particularly \genetic, show more violations of $\varphi$. The improvement of \ltlfbase with larger coverage can be attributed to its use of $o_5$ Eq.~\eqref{eq:conf}, which enables faster convergence and higher \sat.
It is worth noticing %'s noted 
that $\Sigma$ coverage is only one factor influencing counterfactual results: different \LTLf formulae built using the same $\Sigma$ can yield different %varied 
outcomes depending on the %associated 
semantics of the formula $\varphi$, which, in turn, affects its associated \DFA. %associated with $\varphi$. 
The differences among the results of the strategies for the two datasets represent an example of this situation. %One example of this, are the differences between the results between the two datasets. 
For the first dataset, we see that the differences among %between 
the strategies are more pronounced as the coverage increases, while for the second dataset, although %while 
this trend persists, the differences are much less notable.

==> proofs.tex <==

\section{Proofs}
We prove the theorems witnessing correctness of our approach, i.e., that the crossover operator of Algorithm~\ref{alg:crossoveroperator}, as well as the mutation operators by the two strategies of Algorithm~\ref{alg:mutation_operator}, preserve the satisfaction of \LTLp formulae.

\thmalgoone*

\begin{proof}
Let $n = \length(\trace)$.
Upon inspection of Algorithm~\ref{alg:crossoveroperator}, one can see that every output $\trace_o$ produced by the algorithm  relates to the input trace $\trace$ as follows:
\begin{compactenum}
\item $\length(\trace_o) = n$;
\item for every $i \in \set{1,\ldots,n}$:
\begin{compactenum}
\item if $\trace(i) \in \activetasks{\varphi}$ then $\trace_o(i) = \trace(i)$;
\item if instead $\trace(i) \not \in \activetasks{\varphi}$, that is, $\trace(i) \in \othertasks{\varphi}$, then $\trace_o(i) \in \othertasks{\varphi}$ as well or, equivalently $\trace_o(i) \in \othertasks{\varphi}$ if and only if $\trace(i) \in \othertasks{\varphi}$.
\end{compactenum}
\end{compactenum}


By absurdum, imagine that $\trace_o \not \models \varphi$. Since, by property (1) above, $\length(\trace_o) = \length(\trace)$, this means that there exists $i \in \set{1,\ldots,n}$ and an atomic sub-formula $a \in \Sigma$ of $\varphi$ (which, by definition, means $a \in \activetasks{\varphi}$) such that 
either:
\begin{compactenum}[(A)]
\item $\trace,i \models a$ and $\trace_o,i \not \models a$, or 
\item $\trace,i \not\models a$ and $\trace_o,i \models a$. 
\end{compactenum}


\noindent \emph{Case (A).} By \LTLp semantics, we have $\trace(i) = a$ and $\trace_o(i) \neq a$. However, this is impossible: since $a$ belongs to $\activetasks{\varphi}$, then by property (2a) above, we have $\trace(i) = \trace_o(i)$.

\noindent \emph{Case (B).} By the \LTLp semantics, $\trace,i \not \models a$ if and only if $\trace(i) = b$ for some $b \in \Sigma \setminus \set{a}$. There are two sub-cases: either $b \in \activetasks{\varphi}\setminus \set{a}$, or $b \in \othertasks{b}$. In the first sub-case, impossibility follows again from the fact that, by property (2a) above, since $b \in \activetasks{\varphi}$, then $\trace_o(i) = \trace(i) =b$, which implies $\trace_o,i \not\models a$. In the second sub-case, impossibility follows from the fact that $\trace_o(i)$ cannot be $a$, since by property (2b), the fact that $\trace(i) \in \othertasks{b}$ implies that also $\trace_o(i) \in \othertasks{b}$.
\end{proof}


\thmalgothree*

\begin{proof}
The case of \firstheur is proven analogously of Theorem~\ref{thm:crossover}
.
\secondheur
\end{proof}



==> supplementary_material.tex <==
\section{Supplementary material}

\subsection*{Proofs}
We prove the theorems witnessing correctness of our approach, i.e., that the crossover operator of Algorithm~\ref{alg:crossoveroperator}, as well as the mutation operators by the two strategies of Algorithm~\ref{alg:mutation_operator}, preserve the satisfaction of \LTLp formulae.

\thmalgoone*

\begin{proof}
Let $n = \length(\trace)$.
Upon inspection of Algorithm~\ref{alg:crossoveroperator}, one can see that every output $\trace_o$ produced by the algorithm  relates to the input trace $\trace$ as follows:
\begin{compactenum}
\item $\length(\trace_o) = \length(\trace) = n$;
\item for every $i \in \set{1,\ldots,n}$:
\begin{compactenum}
\item if $\trace(i) \in \activetasks{\varphi}$ then $\trace_o(i) = \trace(i)$;
\item if instead $\trace \not \in \activetasks{\varphi}$, that is, $\trace  \in \othertasks{\varphi}$, then $\trace_o(i) \in \othertasks{\varphi}$ as well -- equivalently, $\trace_o(i) \in \othertasks{\varphi}$ if and only if $\trace(i) \in \othertasks{\varphi}$.
\end{compactenum}
\end{compactenum}


By absurdum, imagine that $\trace_o \not \models \varphi$. Since, by property (1) above, $\length(\trace_o) = \length(\trace)$, this means that the violation must occur due to a mismatch in the evaluation of an atomic formula in some instant. Technically, there must exist $i \in \set{1,\ldots,n}$ and an atomic sub-formula $a \in \Sigma$ of $\varphi$ (which, by definition, requires $a \in \activetasks{\varphi}$) such that 
either:
\begin{compactenum}[(A)]
\item $\trace,i \models a$ and $\trace_o,i \not \models a$, or 
\item $\trace,i \not\models a$ and $\trace_o,i \models a$. 
\end{compactenum}


\noindent \emph{Case (A).} By the \LTLp semantics, we have $\trace(i) = a$ and $\trace_o(i) \neq a$. However, this is impossible: since $a$ belongs to $\activetasks{\varphi}$, then by property (2a) above, we have $\trace(i) = \trace_o(i)$.

\noindent \emph{Case (B).} By the \LTLp semantics, $\trace,i \not \models a$ if and only if $\trace(i) = b$ for some $b \in \Sigma \setminus \set{a}$. There are two sub-cases: either $b \in \activetasks{\varphi}\setminus \set{a}$, or $b \in \othertasks{\varphi}$. In the first sub-case, impossibility follows again from the fact that, by property (2a) above, since $b \in \activetasks{\varphi}$, then $\trace_o(i) = \trace(i) =b$, which implies $\trace_o,i \not\models a$. In the second sub-case, impossibility follows from the fact that $\trace_o(i)$ cannot be $a$, since by property (2b), the fact that $\trace(i) \in \othertasks{b}$ implies that also $\trace_o(i) \in \othertasks{b}$.
\end{proof}


\thmalgothree*

\begin{proof}
Correctness of \firstheur is proven analogously of Theorem~\ref{thm:crossover}. Correctness of \secondheur derives directly from the correspondence between the traces that satisfy $\varphi$, and the traces accepted by the \DFA of $\varphi$, $\aut_\varphi$. From the definition of \DFA acceptance, we have that since trace $\trace_o$ satisfies $\varphi$, there is a sequence $\istate, \ldots, \state_{n}$ of states of $\aut_\varphi$, such that:
\begin{inparaenum}[\itshape (i)]
\item the sequence starts from the initial state $\istate$ of $\aut$;
\item the sequence culminates in a last state, that is, $\state_{n} \in \fstates$;
\item for every $i \in \set{1,\ldots,n}$, we have $\trans(q_{i-1},\trace_o(i)) = q_{i}$. 
\end{inparaenum}

From Algorithm~\ref{alg:mutation_operator}, we have that trace $\trace_o$ is mutated through \secondheur by selecting an instant $i$, and allowing for replacing $\trace_o(i)$ with an activity $a$ returned from Algorithm~\ref{alg:safemoves}. From Algorithm~\ref{alg:safemoves}, we know that activity $a$ is returned if the following property holds: $\trans(\state_{i-1},a) = q_{i}$. This means that the mutated trace $\trace'_o$ that replaces $\trace_o(i)$ with $a$, and maintains the rest identical, is accepted by $\aut_\varphi$, with the same witnessing sequence of states $\istate, \ldots, \state_{n}$. From the correspondence between $\aut_\varphi$ and the \LTLp semantics of $\varphi$, we thus have $\trace'_o \models \varphi$.
\end{proof}


\subsection*{Technical material}
\subsubsection{Code for reproducing experiments}

The \emph{AAAI2025-temporal-constrained-counterfactuals} archive contains all the code used for re-running the experiments, including instructions on how to set up the environment and to install all the required dependencies. These instructions are provided in a Markdown file \emph{README.md}, detailing all the steps and commands for installation of all the packages detailed above.


\subsubsection{Code for results analysis}
The analysis of the results generated from the experiments is performed using a separate Jupyter notebook. This notebook includes code for loading and preprocessing the experimental results, performing statistical analysis such as calculating performance metrics, visualizing data, and comparing different methods. It also contains scripts for plotting results to visualize the performance and method comparisons.

This Jupyter notebook is included in the supplementary material and provides a comprehensive view of the analysis conducted, ensuring transparency and reproducibility of our results. For further details, the Jupyter notebook \emph{results\_analysis.ipynb} can be accessed as part of the supplementary material package.


\subsection*{Datasets}
Instructions to download the datasets used to run the experiments above are detailed in the README.MD file in the directory containing the code.

\subsection*{\LTLp formulas for each dataset}

For each dataset, we used different Linear Temporal Logic over Process Traces (\LTLp) formulas to check coverage at 10\%, 25\%, and 50\%. Below are the specific formulas used for each dataset:

\subsubsection*{BPIC2012 Dataset}

\begin{itemize}
    \item \textbf{10\%:}
    $
    \eventually(\text{osentcomplete}) \land \always(\text{osentcomplete} \rightarrow \neg(\text{aacceptedcomplete})\until(\text{wcompleterenaanvraagcomplete})) \land \eventually(\text{osentbackcomplete})
    $
    
    \item \textbf{25\%:}
    $
    \eventually(\text{osentcomplete}) \land \always(\text{osentcomplete} \rightarrow \neg(\text{aacceptedcomplete})\until(\text{wcompleterenaanvraagcomplete})) \land \eventually(\text{osentbackcomplete}) \land \always(\text{wcompleterenaanvraagstart} \rightarrow \eventually(\text{aacceptedcomplete})) \land (\eventually(\text{wnabellenoffertesstart}) \land \eventually(\text{wnabellenoffertescomplete})) \land (\eventually(\text{oselectedcomplete}) \lor \eventually(\text{wvaliderenaanvraagstart}))
    $
    
    \item \textbf{50\%:}
    $
    \eventually(\text{osentcomplete}) \land \always(\text{osentcomplete} \rightarrow \neg(\text{aacceptedcomplete})\until(\text{wcompleterenaanvraagcomplete})) \land \always(\text{wcompleterenaanvraagschedule} \rightarrow \eventually(\text{wcompleterenaanvraagstart})) \land (\eventually(\text{wnabellenoffertesstart}) \lor \eventually(\text{wnabellenoffertescomplete})) \land (\eventually(\text{oselectedcomplete}) \lor \eventually(\text{wvaliderenaanvraagstart})) \land \text{asubmittedcomplete} \land \eventually(\text{oselectedcomplete} \lor \text{apartlysubmittedcomplete}) \land \always(\text{ocreatedcomplete} \rightarrow \eventually(\text{osentbackcomplete})) \land \eventually(\text{afinalizedcomplete}) \lor \eventually(\text{apreacceptedcomplete}) \lor \eventually(\text{wafhandelenleadscomplete})
    $
\end{itemize}

\subsubsection*{BPIC17 Dataset}

\begin{itemize}
    \item \textbf{10\%:}
    $
    \text{acreateapplication} \land \neg(\text{aconcept})\until(\text{wcompleteapplication})
    $
    
    \item \textbf{25\%:}
    $
    \text{acreateapplication} \land \neg(\text{aconcept})\until(\text{wcompleteapplication}) \land (\eventually(\text{ocreateoffer}) \rightarrow \eventually(\text{wcallafteroffers})) \land \eventually(\text{wcompleteapplication})
    $
    
    \item \textbf{50\%:}
    $
    \text{acreateapplication} \land \neg(\text{aconcept})\until(\text{wcompleteapplication}) \land \always(\text{ocreateoffer} \rightarrow (\eventually(\text{wcallafteroffers}) \lor \eventually(\text{wvalidateapplication}))) \land (\eventually(\text{ocreated}) \rightarrow X(\text{osentmailandonline} \lor \text{osentonlineonly})) \land \always((\text{aincomplete} \lor \text{apending}) \rightarrow (X(\text{wcallincompletefiles}) \land \eventually(\text{wvalidateapplication})))
    $
\end{itemize}

\subsubsection*{Claim Management Dataset}

\begin{itemize}
    \item \textbf{10\%:}
    $
    \always(\text{contacthospital} \rightarrow X(\text{acceptclaim} \lor \text{rejectclaim}))
    $
    
    \item \textbf{25\%:}
    $
    \always(\text{contacthospital} \rightarrow X(\text{acceptclaim} \lor \text{rejectclaim})) \land \eventually(\text{createquestionnaire})
    $
    
    \item \textbf{50\%:}
    $
    (\eventually(\text{contacthospital}) \rightarrow \eventually(\text{highinsurancecheck})) \land \always(\text{preparenotificationcontent} \rightarrow X(\text{sendnotificationbyphone} \lor \text{sendnotificationbypost})) \land \always(\text{createquestionnaire} \rightarrow \eventually(\text{preparenotificationcontent})) \land \text{register}
    $
\end{itemize}


\subsection*{Predictive model Hyperparameter Configuration}

For the XGBoost predictive model, we defined the following hyperparameter search space:

\begin{itemize}

    \item The \emph{number of estimators} (\texttt{n\_estimators}) was selected from an integer range between 150 and 1000.

    \item The \emph{maximum} depth of each tree (\texttt{max\_depth}) was chosen as an integer value within the range of 3 to 30.
    
    \item The learning rate (\texttt{learning\_rate}) was selected from a continuous uniform distribution between 0.01 and 0.5.
    
    \item The \emph{subsample} ratio of the training instance (\texttt{subsample}) was chosen from a continuous uniform distribution between 0.5 and 1.    
\end{itemize}

The hyperparameter search was performed using the Hyperopt library, which allowed us to explore this search space efficiently to find the best configuration for our XGBoost model. We ran the hyperparameter search for 20 iterations for each dataset, prefix length and \LTLp combination.



\subsection*{Software and Tools Used for Compliance Checking with \LTLp Formula}

In our experiments, we utilized the \textbf{Declare4Py} Python package, which is available at \texttt{https://github.com/ \ ivanDonadello/Declare4Py}. This package was specifically employed to check compliance with Linear Temporal Logic over Finite Traces (\LTLf) formulas, readily applicable for \LTLp formulas.

The \textbf{Declare4Py} package relies on several external tools to perform its compliance checking:

\begin{enumerate}
    \item \textbf{LTLf2DFA}:
    \begin{itemize}
        \item The \textbf{LTLf2DFA} tool is necessary for converting \LTLp formulas into Deterministic Finite Automata (DFA), which is a crucial step in the compliance checking process.
        \item You can access \textbf{LTLf2DFA} at \texttt{https://github.com/ \ whitemech/LTLf2DFA/}
        \item \textbf{LTLf2DFA} itself has a dependency on the \textbf{MONA} tool.
    \end{itemize}
    
    \item \textbf{MONA}:
    \begin{itemize}
        \item \textbf{MONA} is a C++ package required by \textbf{LTLf2DFA} to handle the conversion process from \LTLp to DFA efficiently.
        \item \textbf{MONA} can be downloaded from \texttt{}{https://www.brics.dk/mona/download.html}.
    \end{itemize}
\end{enumerate}

These tools together enabled the effective compliance checking against the \LTLp formulas in our experimental setup.


\subsection*{Random Seed Settings}
For reproducibility of results in both hyperparameter optimization and counterfactual generation, random seed settings are crucial. In our experiments, we use the following random seed management approaches:

\begin{itemize}
    \item \textbf{Hyperparameter Optimization:} We use random seeds to ensure the reproducibility of the hyperparameter search process. This involves setting a fixed random seed when sampling hyperparameters, which is crucial for obtaining consistent and comparable results across different runs. For instance, we utilize the `np.random.seed(seed\_value)` function from NumPy to control randomness during hyperparameter tuning.
    \item \textbf{Counterfactual Generation:} Random seeds are also used to ensure reproducibility in the counterfactual generation process. This involves setting the random seed for various stochastic elements within the counterfactual generation algorithms. Again, we use `np.random.seed(seed\_value)` to achieve this.
\end{itemize}

The specific random seed values used in our experiments are detailed in the configuration settings of our code.

